RAMP: A Flat Nanosecond Optical Network and MPI Operations for Distributed Deep Learning Systems

Distributed deep learning (DDL) systems strongly depend on network performance. Current electronic packet switched (EPS) network architectures and technologies suffer from variable diameter topologies, low-bisection bandwidth and over-subscription affecting completion time of communication and collective operations. We introduce a near-exascale, full-bisection bandwidth, all-to-all, single-hop, all-optical network architecture with nanosecond reconfiguration called RAMP, which supports large-scale distributed and parallel computing systems (12.8~Tbps per node for up to 65,536 nodes). For the first time, a custom RAMP-x MPI strategy and a network transcoder is proposed to run MPI collective operations across the optical circuit switched (OCS) network in a schedule-less and contention-less manner. RAMP achieves 7.6-171$\times$ speed-up in completion time across all MPI operations compared to realistic EPS and OCS counterparts. It can also deliver a 1.3-16$\times$ and 7.8-58$\times$ reduction in Megatron and DLRM training time respectively} while offering 42-53$\times$ and 3.3-12.4$\times$ improvement in energy consumption and cost respectively.

==> Tables/cost_test.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\setcounter{table}{2}
\definecolor{Gallery}{rgb}{0.937,0.937,0.937}
\begin{table}[b!]
\centering
\caption{Cost estimated for RAMP OCS network compared to current state-of-the-art EPS HPC (SuperPod\cite{superpod}) and DCN (Fat-Tree) networks scaled to 65,536 nodes with matched bandwidth of 12.8Tbps. $\sigma$ represents the intra-to-inter system oversubscription ratio. To match the EPS system node to the RAMP one at 12.8Tbps ($\sigma=1:1$), 64-128 transceivers (200-100 Gbps) per node and 64-128 copies of separate 3-tier Fat-Tree networks are presented for HPC and DCN, respectively. The OCS system uses $x=32$ transceivers each operating at 400Gbps.}
\label{tab:cost}
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[156]Q[65]Q[77]Q[69]Q[79]Q[75]Q[67]Q[81]Q[71]Q[71]Q[113]},
  row{2} = {Gallery,c},
  row{3} = {Gallery,c},
  column{2} = {Gallery},
  cell{1}{1} = {c=2,r=3}{0.221\linewidth},
  cell{1}{3} = {c=2,r=2}{0.146\linewidth,Gallery,c},
  cell{1}{5} = {c=7}{0.557\linewidth,Gallery,c},
  cell{2}{5} = {c=3}{0.221\linewidth},
  cell{2}{8} = {c=3}{0.222\linewidth},
  cell{2}{11} = {r=2}{},
  cell{4}{1} = {r=2}{Gallery},
  cell{4}{3} = {c=2}{0.146\linewidth,c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{4}{7} = {c},
  cell{4}{8} = {c},
  cell{4}{9} = {c},
  cell{4}{10} = {c},
  cell{4}{11} = {c},
  cell{5}{3} = {c=2}{0.146\linewidth,c},
  cell{5}{5} = {c=6}{0.444\linewidth,c},
  cell{5}{11} = {c},
  cell{6}{1} = {c=2}{0.221\linewidth,Gallery},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{6}{7} = {c},
  cell{6}{8} = {c},
  cell{6}{9} = {c},
  cell{6}{10} = {c},
  cell{6}{11} = {c},
  cell{7}{1} = {c=2}{0.221\linewidth,Gallery},
  cell{7}{3} = {c=2}{0.146\linewidth,c},
  cell{7}{5} = {c=6}{0.444\linewidth,c},
  cell{7}{11} = {c},
  cell{8}{1} = {c=4}{0.367\linewidth,Gallery},
  cell{8}{5} = {c=3}{0.221\linewidth,c},
  cell{8}{8} = {c=3}{0.222\linewidth,c},
  cell{8}{11} = {c},
  cell{9}{1} = {c=4}{0.367\linewidth,Gallery},
  cell{9}{5} = {c},
  cell{9}{6} = {c},
  cell{9}{7} = {c},
  cell{9}{8} = {c},
  cell{9}{9} = {c},
  cell{9}{10} = {c},
  cell{9}{11} = {c},
  cell{10}{1} = {c=4}{0.367\linewidth,Gallery},
  cell{10}{5} = {c=3}{0.221\linewidth,c},
  cell{10}{8} = {c=3}{0.222\linewidth,c},
  cell{10}{11} = {c},
  vlines,
  hline{1,4,6-11} = {-}{},
  hline{2} = {5-11}{},
  hline{3} = {3-10}{},
  hline{5} = {2-11}{},
}
                                       &               & {\textbf{Component}\\\textbf{ Cost (\$) }} &              & \textbf{\#items / network} &               &               &                       &               &               &                \\
                                       &               &                                            &              & \textbf{HPC SuperPod \cite{superpod}}         &               &               & \textbf{DCN Fat-Tree} &               &               & \textbf{RAMP } \\
                                       &               & \textbf{EPS}                               & \textbf{DCN} & \textbf{1:1}               & \textbf{10:1} & \textbf{64:1} & \textbf{1:1}          & \textbf{10:1} & \textbf{64:1} &                \\
{\textbf{Transceivers}\\\textbf{ for}} & \textbf{EPS \cite{marc}} & 200                                        &              & 25.2M                      & 2M            & 0.3M          & 50.3M                 & 4.7M          & 0.8M          & -              \\
                                       & \textbf{OCS}  & 600-1200                                   &              & ~-                         &               &               &                       &               &               & 2.1M           \\
\textbf{Switch EPS \cite{mellanox_technologies_qm8790_2021, arista_price_min,arista_price_max}}                  &               & 23,7k                                      & 44k          & 530k                       & 49.7K         & 8.3K          & 655Kk                 & 61.4k         & 10.2k         & -              \\
\textbf{Coupler OCS \cite{PON_cost}}                  &               & 3000                                       &              & -~                         &               &               &                       &               &               & 32.8K          \\
\textbf{Trxs. : Switches cost ratio}   &               &                                            &              & 25:75                      &               &               & 19:81                 &               &               & 93:7,96:4      \\
\textbf{Total Network cost (B\$)}      &               &                                            &              & 16.8                       & 1.57          & 0.26          & 35.5                  & 3.33          & 0.55          & 1.35-2.61      \\
\textbf{Normalised cost (\$/Gbps)}     &               &                                            &              & 20.02                      &               &               & 42.38                 &               &               & 1.62-3.12      
\end{tblr}
}
\end{table}

==> Tables/table_cost.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\setcounter{table}{2}
\begin{table}[!b]

\centering
\caption{Cost estimated for RAMP OCS Networks compared to current state-of-the-art EPS Network at 65536 Nodes with matched bandwidth of 12.8Tbps}
\begin{tabular}{|llc|cc|}
\hline
\multicolumn{2}{|l|}{}                                                                                                                                                                           & \cellcolor[HTML]{EFEFEF}                                                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\#items / network}}                                                                                                                                       \\ \hhline{*2{~}*1{~}*2{-}}
\multicolumn{2}{|l|}{\multirow{-2}{*}{}}                                                                                                                                                         & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Component\\ Cost (\$)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}EPS HPC\\ Fat-Tree\end{tabular}}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}} RAMP\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}}                                                                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{EPS\cite{marc}}} & 200                                                                                                                  & \multicolumn{1}{c|}{21299200}                                                                                      & -                                                                                        \\ \hhline{|>{\arrayrulecolor{gray!15}}->{\arrayrulecolor{black}}|--|->{\arrayrulecolor{black}}|->{\arrayrulecolor{black}}|}
\multicolumn{1}{|l|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}Transceivers \\ for\end{tabular}}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{OCS}} & 300-600                                                                                                             & \multicolumn{1}{c|}{-}                                                                                           & 2097152                                                                                  \\ \hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Switch for EPS \cite{Nvidia_switch_cost}}}                                                                                                                            & 23,698                                                                                                                  & \multicolumn{1}{c|}{532480}                                                                                        & -                                                                                        \\ \hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Coupler for OCS \cite{PON_cost}}}                                                                                                                           & 3000                                                                                                                  & \multicolumn{1}{c|}{-}                                                                                           & 32768                                                                                    \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Transceiver : Switch cost ratio}}                                                                                                                                                                                                                                   & \multicolumn{1}{c|}{25:75}                                                                                       & 93:7,98:2                                                                                      \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Network cost (B\$)}}                                                                                                                                                                                                                                            & \multicolumn{1}{c|}{16.88}                                                                                       & 0.7-1.35B                                                                                \\ \hline
\multicolumn{3}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Normalised Network cost (\$/Gb)}}                                                                                                                                                                                                                                            & \multicolumn{1}{c|}{20.12}                                                                                       & 0.87-1.62                                                                                \\ \hline
\end{tabular}
\label{tab:cost}

\end{table}

==> Tables/table_related_work.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tp]

\centering
\caption{{RAMP with respect to Current leading  OCS networks for DDL Systems}}
\label{related_table}

\begin{tabular}{|c|c|c|c|c|c|}
\hline
                                                                                            & \cellcolor[HTML]{EFEFEF}\textbf{{\#Nodes}} & \cellcolor[HTML]{EFEFEF}\textbf{{\begin{tabular}[c]{@{}c@{}}All-to-all\\  Connect.\end{tabular}}} & \cellcolor[HTML]{EFEFEF}\textbf{{\begin{tabular}[c]{@{}c@{}}N2N\\  Capacity \\ (Tbps)\end{tabular}}} & \cellcolor[HTML]{EFEFEF}\textbf{{\begin{tabular}[c]{@{}c@{}}   Circuit\\  reconfig.\end{tabular}}} & \cellcolor[HTML]{EFEFEF}\textbf{{\begin{tabular}[c]{@{}c@{}}   Supports\\   Link \\   Failure\end{tabular}}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Sip-ML \\  OCS\end{tabular}}     & {\color[HTML]{000000} O(1000)}        & Yes                                                                                                 & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}8.2\end{tabular}}           & {\color[HTML]{000000} 10~ms}                                                                    & \begin{tabular}[c]{@{}c@{}}Yes\end{tabular}                                                               \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Sip-ML\\  TeraRack\end{tabular}} & {\color[HTML]{000000} 256}          & {\color[HTML]{000000} No}                                                                  & {\color[HTML]{000000} 2.4}                                                                      & {\color[HTML]{000000} 25~$\mu$s}                                                                                                    & {\color[HTML]{000000} No}                                                                                  \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{\textsc{TopoOpt}}                                                    & {\color[HTML]{000000} 384}          & Yes                                                                                                 & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}0.2\end{tabular}}              & {\color[HTML]{000000} 10~ms}                                                                    & \begin{tabular}[c]{@{}c@{}}Yes\end{tabular}                                                               \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Sirius}                                                     & N/A                                        & Yes                                                                                                 & {\color[HTML]{000000} 0.4}                                                                      & O(ns)                                                                                  & {\color[HTML]{000000} No}                                                                                  \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{PULSE}                                                      & 65536                                        & Yes                                                                                                 & {\color[HTML]{000000} 0.4}                                                                      & O(ns)                                                                                      & {\color[HTML]{000000} No}                                                                                  \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{RAMP}                                                       & \textbf{65536}                               & \textbf{Yes}                                                                                        & \textbf{12.8}                                                                                            & \textbf{O(ns)}                                                                                    & \textbf{\begin{tabular}[c]{@{}c@{}}Yes\end{tabular}}                                                 \\ \hline
\end{tabular}

\end{table}

==> Tables/test_2_tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% \begin{wraptable}[h]
\setcounter{table}{5}

\begin{table*}[bp]

\mbox{}
\hfill
  \begin{minipage}[t]{.7\linewidth}
 \centering
\caption{Message size and operations per algorithmic step for different collective operations}
\begin{tabular}{ll|llll|ll|}
\cline{3-8}
\hhline{*2{~}*6{-}}
 &
   &
  \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}Message size per step ($m=$ original message size)} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}Local Ops.} \\ \cline{3-8}
  \hhline{*2{~}*6{-}}
 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}2} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}3} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}4} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}Op.} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}Buff\_Op} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} &
  \cellcolor[HTML]{C0C0C0}Red.-Scatter &
  \multicolumn{1}{l|}{$m/x$} &
  \multicolumn{1}{l|}{$m/x^2$} &
  \multicolumn{1}{l|}{$m/(Jx^2)$} &
  $m/(J\Lambda x)$ &
  \multicolumn{1}{l|}{Reduce} &
  Reshape \\ \cline{2-8} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} &
  \cellcolor[HTML]{C0C0C0}All-Gather &
  \multicolumn{1}{l|}{$m \cdot \Lambda/x$} &
  \multicolumn{1}{l|}{$m \cdot J \Lambda/x$} &
  \multicolumn{1}{l|}{$m \cdot J \Lambda$} &
  $m \cdot J \Lambda x$ &
  \multicolumn{1}{l|}{Identity} &
  Copy \\ \cline{2-8} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} &
  \cellcolor[HTML]{C0C0C0}Barrier &
  \multicolumn{1}{l|}{$0$} &
  \multicolumn{1}{l|}{$0$} &
  \multicolumn{1}{l|}{$0$} &
  $0$ &
  \multicolumn{1}{l|}{Logical and} &
  Identity \\ \cline{2-8} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} &
  \cellcolor[HTML]{C0C0C0}All-to-All &
  \multicolumn{1}{l|}{$m/x$} &
  \multicolumn{1}{l|}{$m/x$} &
  \multicolumn{1}{l|}{$m/J$} &
  $m \cdot x/\Lambda$ &
  \multicolumn{1}{l|}{Reshape} &
  Reshape \\ \cline{2-8} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} &
  \cellcolor[HTML]{C0C0C0}Scatter &
  \multicolumn{1}{l|}{$m/x$} &
  \multicolumn{1}{l|}{$m/x^2$} &
  \multicolumn{1}{l|}{$m/(Jx^2)$} &
  $m/(J\Lambda x)$ &
  \multicolumn{1}{l|}{Identity} &
  Reshape \\ \cline{2-8} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}} &
  \cellcolor[HTML]{C0C0C0}Gather &
  \multicolumn{1}{l|}{$m \cdot \Lambda/x)$} &
  \multicolumn{1}{l|}{$m \cdot J \Lambda/x$} &
  \multicolumn{1}{l|}{$m \cdot J \Lambda$} &
  $m \cdot J \Lambda x$ &
  \multicolumn{1}{l|}{Identity} &
  Copy \\ \cline{2-8} 
\multicolumn{1}{|l|}{\multirow{-7}{*}{\cellcolor[HTML]{EFEFEF}{\rotatebox[origin=c]{90}{\footnotesize{MPI Operations}}}}} &
  \cellcolor[HTML]{C0C0C0}Broadcast &
  \multicolumn{4}{l|}{$m/k$ for $s+k-2$s steps} &
  \multicolumn{1}{l|}{Identity} &
  Identity \\ \hline
\end{tabular}
\label{tab:collective_info}
\end{minipage}\hfill
\begin{minipage}[t]{.27\linewidth}
\centering
\caption{Formula describing what portion of the previous message should be received by a node at any algorithmic step.}
\begin{tabular}{|l|l|}
\hline
\hhline{*2{-}}
\rowcolor[HTML]{EFEFEF} Step & Information portion formula                                    \\ \hline
\multirow{2}{*}{1}           & $\left( g  - \lambda - j - \floor{\lambda/x}j \right) $        \\
                             & $\textrm{mod } x$                                              \\ \hline
2                            & $\left(  g  - j - \floor{\lambda/x}j \right) \textrm{ mod } x$ \\ \hline
3                            & $j$                                                            \\ \hline
4                            & $\floor{\lambda/x}$                                            \\ \hline
\end{tabular}
\label{tab:reduce-info}
\end{minipage}\hfill

\end{table*}
% }

% \end{wraptable}




